Deductron -- A Recurrent Neural Network

The current paper is a study in Recurrent Neural Networks (RNN), motivated by the lack of examples simple enough so that they can be thoroughly understood theoretically, but complex enough to be realistic. We constructed an example of structured data, motivated by problems from image-to-text conversion (OCR), which requires long-term memory to decode. Our data is a simple writing system, encoding characters 'X' and 'O' as their upper halves, which is possible due to symmetry of the two characters. The characters can be connected, as in some languages using cursive, such as Arabic (abjad). The string 'XOOXXO' may be encoded as '${\vee}{\wedge}\kern-1.5pt{\wedge}{\vee}\kern-1.5pt{\vee}{\wedge}$'. It follows that we may need to know arbitrarily long past to decode a current character, thus requiring long-term memory. Subsequently we constructed an RNN capable of decoding sequences encoded in this manner. Rather than by training, we constructed our RNN "by inspection", i.e. we guessed its weights. This involved a sequence of steps. We wrote a conventional program which decodes the sequences as the example above. Subsequently, we interpreted the program as a neural network (the only example of this kind known to us). Finally, we generalized this neural network to discover a new RNN architecture whose instance is our handcrafted RNN. It turns out to be a 3 layer network, where the middle layer is capable of performing simple logical inferences; thus the name "deductron". It is demonstrated that it is possible to train our network by simulated annealing. Also, known variants of stochastic gradient descent (SGD) methods are shown to work.

==> TAGS <==

deductron_paper.tex,7425
\definecolor{inecolor25,434
\definecolor{inecolor26,473
\definecolor{inecolor27,509
\definecolor{inecolor45,924
\definecolor{inecolor46,961
\definecolor{inecolor47,997
\newcommand*\@lbracket{*\@lbracket66,1564
\newcommand*\@rbracket{*\@rbracket67,1590
\newcommand*\@colon{*\@colon68,1616
\newcommand*\colorIndex{*\colorIndex69,1639
\def\complex{\complex83,1925
\def\reals{\reals84,1950
\def\tr{\tr85,1973
\def\interior{\interior86,1994
\newcommand{\DensOps}\DensOps100,2368
\newcommand{\Herm}\Herm101,2408
\newcommand{\SkewHerm}\SkewHerm102,2442
\newcommand{\conv}\conv103,2484
\newcommand{\vect}\vect104,2518
\newcommand*{*115,2811
\def\ALG@printindent{\ALG@printindent118,2980
\newcommand{\elementfun}\elementfun146,4055
\renewcommand{\P}\P147,4098
\newcommand{\e}\e148,4159
\algnewcommand{\Goto}[1]{\algorithmicgoto~\ref{#1}}%159,4533
\section{Introduction}Introduction225,7438
recognition \cite{lstm,journals/neco/GersSC00}lstm,journals/neco/GersSC00254,9136
Tensorflow \cite{tensorflow2015-whitepaper}tensorflow2015-whitepaper336,13538
used the \emph{Adam optimizer} \cite{2014arXiv1412.6980K}2014arXiv1412.6980K339,13744
\section{The W-language  and writing system}The347,14101
Figure~\ref{fig:sample1}fig:sample1357,14523
    'XOOXXO'.\label{fig:sample1}fig:sample1364,14704
could look like Figure~\ref{fig:sample2}fig:sample2370,14957
    string 'XOOXXO'.\label{fig:sample2}fig:sample2384,15434
something like Figure~\ref{fig:sample3}fig:sample3388,15559
\cite{citeulike:141092}citeulike:141092391,15742
    string 'XOOXXO', with some errors.\label{fig:sample3}fig:sample3398,15938
of calligraphy of our messages, as illustrated by Figure~\ref{fig:sample1}fig:sample1408,16472
Figure~\ref{fig:binary-image}fig:binary-image421,17111
\def\pixels{\pixels423,17144
  \definecolor{inecolor431,17395
  \definecolor{inecolor432,17433
  \caption{Binary image of the message 'XOOXXO'.\label{fig:binary-image}fig:binary-image443,17732
In Figure~\ref{fig:raw-bits}fig:raw-bits445,17819
  \caption{Binary image of the message 'XOOXXO' as raw bits.\label{fig:raw-bits}fig:raw-bits456,18155
long.  However, a picture like Figure~\ref{fig:sample4}fig:sample4460,18321
  \caption{A wave.\label{fig:sample4}fig:sample4469,18701
Thus decoding an image like Figure~\ref{fig:sample2}fig:sample2472,18755
Figure~\ref{fig:topological-markov-chain}fig:topological-markov-chain510,20700
    \label{fig:topological-markov-chain}fig:topological-markov-chain562,22964
  Figure~\ref{fig:topological-markov-chain}fig:topological-markov-chain566,23098
\section{A conventional W-language decoding algorithm}A578,23664
In order to correctly decode an image like in Figure~\ref{fig:binary-image}fig:binary-image585,24039
look like Algorithm~\ref{alg:basic-decoding}alg:basic-decoding673,27026
    representing a sequence of 'X' and 'O'. \label{alg:basic-decoding}alg:basic-decoding680,27371
    Algorithm~\ref{alg:basic-decoding}alg:basic-decoding712,28873
  Design a similar algorithm to Algorithm~\ref{alg:basic-decoding}alg:basic-decoding716,29028
  Algorithm~\ref{alg:basic-decoding}alg:basic-decoding723,29358
\section{Converting a conventional program to a neural net}Converting733,29665
The conditions in Algorithm~\ref{alg:basic-decoding}alg:basic-decoding748,30463
We obtain Algorithm~\ref{alg:basic-decoding-arithmetical}alg:basic-decoding-arithmetical774,31358
    arithmetic.\label{alg:basic-decoding-arithmetical}alg:basic-decoding-arithmetical780,31615
Algorithm~\ref{alg:basic-decoding-arithmetical}alg:basic-decoding-arithmetical806,32943
This results in Algorithm~\ref{alg:basic-decoding-arithmetical-final}alg:basic-decoding-arithmetical-final808,33054
    neurons.\label{alg:basic-decoding-arithmetical-final}alg:basic-decoding-arithmetical-final816,33456
as Algorithm~\ref{alg:basic-decoding-arithmetical-clean}alg:basic-decoding-arithmetical-clean857,35128
    format.\label{alg:basic-decoding-arithmetical-clean}alg:basic-decoding-arithmetical-clean863,35394
\section{An analysis of the U-gate and a new V-gate}An885,36667
  In this example, we consider Algorithm~\ref{alg:basic-decoding-arithmetical-final}alg:basic-decoding-arithmetical-final976,40465
Algorithm~\ref{alg:three-layer-final}alg:three-layer-final1002,41522
    memory cells.\label{alg:three-layer-final}alg:three-layer-final1012,42098
  Algorithm~\ref{alg:basic-decoding}alg:basic-decoding1052,44064
  Figure~\ref{fig:topological-markov-chain}fig:topological-markov-chain1055,44223
Figure~\ref{fig:deductron}fig:deductron1088,45955
    $b_2$. \label{fig:deductron}fig:deductron1107,46917
    $V(z, u, v)=(1-u)(1-v)z + u$.\label{alg:v-gate}alg:v-gate1134,47923
algorithm, Algorithm~\ref{alg:architecture-simulator}alg:architecture-simulator1143,48197
Figure~\ref{fig:deductron}fig:deductron1146,48327
Algorithm~\ref{alg:architecture-simulator}alg:architecture-simulator1148,48437
    network.\label{alg:architecture-simulator}alg:architecture-simulator1154,48659
\section{Interpretability of the weights as logic formulas}Interpretability1183,49851
    Fig~\ref{fig:binary-image}fig:binary-image1198,50658
In Table~\ref{fig:learned-weights}fig:learned-weights1204,50802
    (Algorithm~\ref{alg:basic-decoding-arithmetical-final}alg:basic-decoding-arithmetical-final1230,52265
    \label{fig:hand-coded-weights}fig:hand-coded-weights1231,52326
Algorithm~\ref{alg:architecture-simulator}alg:architecture-simulator1237,52445
Algorithm~\ref{alg:basic-decoding-arithmetical-final}alg:basic-decoding-arithmetical-final1239,52578
  \label{thm:arithmetic-vs-logic}thm:arithmetic-vs-logic1253,53245
  Prove that under the assumptions of Lemma~\ref{thm:arithmetic-vs-logic}thm:arithmetic-vs-logic1277,54050
\section{Machine learning}Machine1283,54233
Figure~\ref{fig:sample2}fig:sample21293,54690
  \label{eqn:falling-sigmoid}eqn:falling-sigmoid1315,55794
with a graph portrayed in Figure~\ref{fig:falling-sigmoid}fig:falling-sigmoid1319,55884
    for $\beta=5$ and $\beta=15$.\label{fig:falling-sigmoid}fig:falling-sigmoid1323,56036
in Figure~\ref{fig:learned-weights}fig:learned-weights1344,56802
Figure~\ref{fig:learned-weights-output}fig:learned-weights-output1349,57015
Algorithm~\ref{alg:basic-decoding-arithmetical-final}alg:basic-decoding-arithmetical-final1351,57115
Figure~\ref{fig:hand-coded-weights}fig:hand-coded-weights1352,57176
Figure~\ref{fig:topological-markov-chain}fig:topological-markov-chain1356,57453
  \caption{\label{fig:learned-weights-output}fig:learned-weights-output1364,57834
    optimal weights constructed by simulated annealing (Figure~\ref{fig:learned-weights}fig:learned-weights1365,57913
    for input depicted in Figure~\ref{fig:binary-image}fig:binary-image1367,58078
\section{Continuous weights}Continuous1403,59915
  \label{eqn:rising-sigmoid}eqn:rising-sigmoid1412,60350
  \label{eqn:loss-function}eqn:loss-function1420,60596
  Using Figure~\ref{fig:deductron}fig:deductron1425,60765
    \frac{\partial\, loss}ial\,1429,60973
    \frac{\partial\, loss}ial\,1430,61028
The system Tensorflow \cite{tensorflow2015-whitepaper}tensorflow2015-whitepaper1443,61751
of a deductron RNN, closely following Figure~\ref{fig:deductron}fig:deductron1450,62153
\section{Conclusions}Conclusions1453,62291
\appendix1483,63640

lstm.tex,145
\section{Peephole LSTM Architecture}Peephole2,1
\label{appendix:LSTM}appendix:LSTM3,38
the following diagram (\cite{wiki:xxx}wiki:xxx5,106

python.tex,444
\section{Python codes}Python1,0
\label{appendix:python}appendix:python2,23
\subsection{A simple Deductron simulator}A9,330
\subsection{Training implemented in Python}Training25,1062
The output is illustrated in Figure~\ref{fig:learned-weights}fig:learned-weights43,2041
\subsection{Training implemented in Tensorflow}Training45,2105
The following Python/Tensorflow \cite{tensorflow2015-whitepaper}tensorflow2015-whitepaper46,2153

_region_.tex,966
\definecolor{inecolor25,471
\definecolor{inecolor26,510
\definecolor{inecolor27,546
\definecolor{inecolor45,961
\definecolor{inecolor46,998
\definecolor{inecolor47,1034
\newcommand*\@lbracket{*\@lbracket66,1601
\newcommand*\@rbracket{*\@rbracket67,1627
\newcommand*\@colon{*\@colon68,1653
\newcommand*\colorIndex{*\colorIndex69,1676
\def\complex{\complex83,1962
\def\reals{\reals84,1987
\def\tr{\tr85,2010
\def\interior{\interior86,2031
\newcommand{\DensOps}\DensOps100,2405
\newcommand{\Herm}\Herm101,2445
\newcommand{\SkewHerm}\SkewHerm102,2479
\newcommand{\conv}\conv103,2521
\newcommand{\vect}\vect104,2555
\newcommand*{*115,2848
\def\ALG@printindent{\ALG@printindent118,3017
\newcommand{\elementfun}\elementfun146,4092
\renewcommand{\P}\P147,4135
\newcommand{\e}\e148,4196
\algnewcommand{\Goto}[1]{\algorithmicgoto~\ref{#1}}%159,4570
    memory cells.\label{alg:three-layer-final}alg:three-layer-final196,5586

ugate.tex,164
\section{Our architecture with U-gate}Our1,0
Figure~\ref{fig:uarchitecture}fig:uarchitecture3,102
  \caption{\label{fig:uarchitecture}fig:uarchitecture10,318

three_layer.tex,0

tdiag.tex,0

deductron.tex,0

